Read Anywhere Pointed: Layout-aware GUI Screen Reading with Tree-of-Lens Grounding

Graphical User Interfaces (GUIs) are central to our interaction with digital devices and growing efforts have been made to build models for various GUI understanding tasks. However, these efforts largely overlook an important GUI-referring task: screen reading based on user-indicated points, which we name the Screen Point-and-Read (ScreenPR) task. Currently, this task is predominantly handled by rigid accessible screen reading tools, in great need of new models driven by advancements in Multimodal Large Language Models (MLLMs). In this paper, we propose a Tree-of-Lens (ToL) agent, utilizing a novel ToL grounding mechanism, to address the ScreenPR task. Based on the input point coordinate and the corresponding GUI screenshot, our ToL agent constructs a Hierarchical Layout Tree. Based on the tree, our ToL agent not only comprehends the content of the indicated area but also articulates the layout and spatial relationships between elements. Such layout information is crucial for accurately interpreting information on the screen, distinguishing our ToL agent from other screen reading tools. We also thoroughly evaluate the ToL agent against other baselines on a newly proposed ScreenPR benchmark, which includes GUIs from mobile, web, and operating systems. Last but not least, we test the ToL agent on mobile GUI navigation tasks, demonstrating its utility in identifying incorrect actions along the path of agent execution trajectories. Code and data: https://screen-point-and-read.github.io

==> tables/table_example.tex <==
% Yue's reference example 1

\begin{table}[t]
    \centering
\setlength{\abovecaptionskip}{0.1cm}
\setlength\tabcolsep{0pt}
\resizebox{\columnwidth}{!}{
\begin{tabular}{llc|c|cc} 
\toprule
% && \multicolumn{8}{|c|}{\textbf { Seen Validation }} & \multicolumn{8}{|c|}{\textbf { Unseen Validation }}& \multicolumn{8}{c}{\textbf { Unseen Testing }} \\
% \hline \multicolumn{1}{r}{\textbf{Task}} 
\multicolumn{3}{c|}{}& \multicolumn{1}{c|}{$\begin{array}{c}
     \textbf{Task}  \\
     \textbf{Completion}
\end{array}$} & \multicolumn{2}{c}{$\begin{array}{c}
     \textbf{Subjective}  \\
     \textbf{Response Evaluation}
\end{array}$}\\
 \cmidrule(lr){4-4} 
 \cmidrule(lr){5-6} 

\multicolumn{2}{c|}{\textbf{Helper}} &
\multicolumn{1}{c|}{$\begin{array}{c}
     \textbf{Task}\\
     \textbf{Performer}
\end{array}$}
& \multicolumn{1}{c|}{$\begin{array}{c}
     \text{GP}\uparrow
\end{array}$}
& \multicolumn{1}{c}{$\begin{array}{c}
     \text{Naturalness}\uparrow
\end{array}$} & \multicolumn{1}{c}{$\begin{array}{c}
     \text{Faithfulness}\uparrow
\end{array}$}\\
\midrule
%  & \text{Rule-based}  & 4.0  & 4.1   &  5.3   & 0.80  & 0.0  & 0.0  & 0.80   & 0.80  & 5.6 & 5.8 & 1.6 & 0.80 & 0.5 &0.5 & 5.1 & 0.81 & 3.4 & 3.6 & 3.3 & 0.80 & 0.0 & 0.0 & 3.3 & 0.82 \\
% \cmidrule(lr){0-1}
\multicolumn{2}{l|}{$\begin{array}{l}
    \text{No helper}\\
\end{array}$} & \multirow{4}{*}{$\begin{array}{l}
    \text{Human}
\end{array}$}  & 3.54 & - & -  \\
% \cmidrule(lr){0-1}
% \cmidrule(lr){4-7}

 \multicolumn{2}{l|}{$\begin{array}{c}
    \text{RMM }\mathcal{G}
\end{array}$} &  & 6.32 & 73/100 & 59/100  \\
% \multicolumn{2}{l|}{$\begin{array}{c}
%     \text{Multimodal LLM}
% \end{array}$} &  &  &  &  &  \\
\multicolumn{2}{l|}{$\begin{array}{l}
    \text{Multi-modal LLM}\\
\end{array}$} &  &  8.44 &  \textbf{75/100} & 60/100 \\

 \multicolumn{2}{l|}{$\begin{array}{l}
    \text{SeeRee}\\
\end{array}$} &  &  \textbf{9.89} &  72/100 & \textbf{75/100}  \\
% \midrule
% $\begin{array}{r}
%     \text {Human}\\
% \end{array}$   & \multicolumn{2}{c}{5.13}  & \multicolumn{2}{c}{5.13} & \multicolumn{2}{c}{0.49} & \multicolumn{2}{c}{0.33}   \\

\bottomrule
\end{tabular}
}
\caption{Results of human evaluation on RdI task on the CVDN \cite{thomason2020vision}. The human tester plays the task performer role via an interface interacting with the helper agents. Task completion and subjective response evaluation are collected. The response from SeeRee is most effective despite being less natural. 
%start in initialized positions and will be provided with target objects based on validation data from CVDN. Different helper agents are tested on the same set of data, and we measure the task completion of human testers, as well as the subjective evaluation on the responses.
%\xin{Is this conducted on R2R or CVDN? Please cite the right paper.}
 \label{tab:table_2} }
% \vspace{-3mm}
\end{table}










\begin{table*}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc}
\toprule
\multicolumn{1}{l|}{} & \multicolumn{2}{c|}{\textbf{Content Description Acc} $\uparrow$}               & \multicolumn{2}{c|}{\textbf{Layout Description Acc} $\uparrow$}                & \multicolumn{2}{c}{\textbf{Verboseness} $\downarrow$}                      \\ 
\cline{2-7}
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{SPR} & \multicolumn{1}{c|}{Human} & \multicolumn{1}{c|}{SPR} & \multicolumn{1}{c|}{Human} & \multicolumn{1}{c|}{Avg Length} & Human  \\ 
\hline
CoL            &                               &                            &                               &                            &                                             &        \\
CoL w/ SoM            &                               &                            &                               &                            &                                             &        \\
Human                &                               &                            &                               &                            &                                             &        \\
CoL w/ GT local regions              &                               &                            &                               &                            &                                             &        \\
CoL w/ GT global regions            &                               &                            &                               &                            &                                             &        \\
CoL w/ GT global and local regions            &                               &                            &                               &                            &                                             &        \\
\bottomrule
\end{tabular}}
\label{table:ablation_0}
\caption{}
\end{table*}





==> tables/text_prompt______example.tex <==
\begin{table}[t]
    \centering


\begin{minipage}[t]{0.5\textwidth}
\subfloat[]{

    \resizebox{\linewidth}{!}{
    \begin{tabular}{llll}
    \toprule
        \multicolumn{4}{m{11cm}}{
          $\begin{array}{rl}
              \textbf{Prompt:} & \text{For question: }\{question\}\\
& \text{Compare the following answers:} \\
& \text{Text 1: } \{output\}\\
& \text{Text 2: } \{gt\}\\
& \text{Does the first one contain all key information in the second}\\
& \text{one? (yes/no)}\\
& \text{Answer:} \\

            
              
          \end{array}$
       }\\
         \bottomrule
    \end{tabular}}


}
\end{minipage}
\begin{minipage}[t]{0.5\textwidth}
\subfloat[]{

    \resizebox{\linewidth}{!}{
    \begin{tabular}{llll}
    \toprule
        \multicolumn{4}{m{11cm}}{
          $\begin{array}{rl}
              \textbf{Prompt:} & \text{\space \space \space \space For question: }\{question\}\\
& \text{\space \space \space \space Ground truth: } \{gt\}\\
& \text{\space \space \space \space Model predicted answer: } \{output\}\\
& \text{\space \space \space \space Based on the question and the ground truth answer, is the }\\
& \text{model's predicted answer correct? If multi-choice is provided, }\\
& \text{think about which choice is selected by the model, is it }\\
& \text{correct? (please answer yes/no)}
          \end{array}$
       }\\
         \bottomrule
    \end{tabular}}
}
\end{minipage}

    \caption{Text prompt for GPT-4 as an evaluator to judge if the output from the model $\{output\}$ is correct given the question $\{question\}$ ground truth answer $\{gt\}$. (a) shows the prompt for GPT-4 to evaluate the model output for the first and second types of question (Q1 and Q2) in MultipanelVQA. (b) shows the prompt for GPT-4 to judge the third type of question (Q3) in MultipanelVQA }



    \label{tab:appendix_evalu_prompt}
\end{table}

\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{llll}
    \toprule
        \multicolumn{4}{m{25cm}}{
          $\begin{array}{rl}
              \textbf{Prompt:} &
\text{\space \space \space \space You are asking questions about an multi-panel image composition with multiple subfigures. You will be given a description of the} \\

& \text{overall layouts of the subfigures, a common question and answers to this question for each subfigure.} \\
            
& \text{\space \space \space \space First ask three questions (Q1, Q2, Q3) and then generate ground truth answers (A1, A2, A3) to each question.} \\

& \text{\space \space \space \space The second question (Q2) should be the same as the common question provided but specifically targeting at one subfigure. Make sure to include} \\
& \text{specific position of the subfigure targeted. } \\
& \text{\space \space \space \space The first question (Q1) asks if all or any subfigures have the specific object/attribute mentioned in Q2. (e.g. Do all the subfigures}\\
& \text{share certain object? Is there any subfigure that has a certain object?). }\\
& \text{\space \space \space \space For both answers A1 and A2, try not to refer to specific positions of subfigures and be concise.}\\

& \text{\space \space \space \space For the third question (Q3) make it a multi-choice question with a single answer based on the common question and answer. The answer (A3)}\\
& \text{should only be the subfigure targeted.} \\ 
& \text{\space \space \space \space Also generate a,b,c,d four choices and randomly put the correct answer in one of them, and fill the other choices with x. }\\
& \text{\space \space \space \space For the third answer (A3), only put in the label for the correct choice (a,b,c or d).
Ask questions only based on the direct information you}\\
& \text{get from the provided common question and answers.}\\
& \text{\space \space \space \space At the end of each question (Q1, Q1 or Q3), indicate what kind of answer is needed for the question. (eg. please answer yes/no, please select one).}\\
& \text{\space \space \space \space Answers generated should be consice without any explanation.}\\
& \text{\space \space \space \space Your output should be in the following format: Q1: A1: 
Q2: 
A2: 
Q3: 
A3: } \\
& \text{\space \space \space \space There are } {\{num\_subfigure\}}\text{ subfigures in the image. The common question for all subfigures are: }\{com\_question\} \text{.}\\
& \text{\space \space \space \space The answer from the target subfigure is: }\{answer\_target\_subfigure\} \text{.} \\
& \text{\space \space \space \space The answer for the other subfigures are not the same as the target subfigure. Ask questions about the target subfigure located at }\{pos\_description\} \text{.}\\
              
          \end{array}$
       }\\
         \bottomrule
    \end{tabular}}
    \caption{Text prompts for generating questions and answers of multipanel images in the synthetic subset of MultipanelVQA benchmark. $\{num\_subfigure\}$ is the number of subfigures in the multipanel image. $\{com\_question\}$ is the common question in the image set from source datasets. $\{answer\_target\_subfigure\}$ is the answer of the target subfigure to the common question, which is different from the answer from the other subfigures selected. $\{pos\_description\}$ is the position description for the target subfigure predefined by human. }
    \label{tab:appendix_prompt_llm}
\end{table*}
